SecretBench: A Dataset of Software Secrets

According to GitGuardian's monitoring of public GitHub repositories, the exposure of secrets (API keys and other credentials) increased two-fold in 2021 compared to 2020, totaling more than six million secrets. However, no benchmark dataset is publicly available for researchers and tool developers to evaluate secret detection tools that produce many false positive warnings. The goal of our paper is to aid researchers and tool developers in evaluating and improving secret detection tools by curating a benchmark dataset of secrets through a systematic collection of secrets from open-source repositories. We present a labeled dataset of source codes containing 97,479 secrets (of which 15,084 are true secrets) of various secret types extracted from 818 public GitHub repositories. The dataset covers 49 programming languages and 311 file types.

==> Tables/secret-regex-list.tex <==
\newcolumntype{e}{>{\hsize=0.02\hsize}X}
\newcolumntype{s}{>{\hsize=0.18\hsize}X}
\newcolumntype{b}{>{\hsize=0.80\hsize}X}
\begin{table} [!htb]
%\small
\footnotesize
\caption{List of Regex Patterns to filter GitHub repositories.}
\label{regex-list}
\begin{tabularx}{\columnwidth} {|e | s | b |}
 \hline
 \multicolumn{1}{|c|}{\textbf{ID}} &
  \multicolumn{1}{c|}{\textbf{Secret Type}} &
  \multicolumn{1}{c|}{\textbf{Regular Expression}}\\
 \hline \hline
 65 & AWS API Secret & \verb/\b([A-Za-z0-9+/]{40})[ \r\n'"\x60]/ \\ \hline
 71 & Azure Client Secret & \verb/(?i)(%s).{0,20}([a-z0-9_\.\-~]{34})/ \\ \hline
 278 & Generic Pattern & \verb/(?i)(?:pass|token|cred|secret|key)(?:.|[\n\r]){0,40}(\b[\x21-\x7e]{16,64}\b)/ \\ \hline
 605 & Slack Token &  \verb/(xoxb$\vert$xoxp$\vert$xapp$\vert$xoxa$\vert$xoxr)-[0-9]10,13[a-zA-Z0-9]*/ \\ \hline
 640 & Stripe API Key & \verb/[rs]k_live_[a-zA-Z0-9]{20,30}/ \\ \hline
\end{tabularx}
\end{table}
